ODExAI: A Comprehensive Object Detection Explainable AI Evaluation

Explainable Artificial Intelligence (XAI) techniques for interpreting object detection models remain in an early stage, with no established standards for systematic evaluation. This absence of consensus hinders both the comparative analysis of methods and the informed selection of suitable approaches. To address this gap, we introduce the Object Detection Explainable AI Evaluation (ODExAI), a comprehensive framework designed to assess XAI methods in object detection based on three core dimensions: localization accuracy, faithfulness to model behavior, and computational complexity. We benchmark a set of XAI methods across two widely used object detectors (YOLOX and Faster R-CNN) and standard datasets (MS-COCO and PASCAL VOC). Empirical results demonstrate that region-based methods (e.g., D-CLOSE) achieve strong localization (PG = 88.49%) and high model faithfulness (OA = 0.863), though with substantial computational overhead (Time = 71.42s). On the other hand, CAM-based methods (e.g., G-CAME) achieve superior localization (PG = 96.13%) and significantly lower runtime (Time = 0.54s), but at the expense of reduced faithfulness (OA = 0.549). These findings demonstrate critical trade-offs among existing XAI approaches and reinforce the need for task-specific evaluation when deploying them in object detection pipelines. Our implementation and evaluation benchmarks are publicly available at: https://github.com/Analytics-Everywhere-Lab/odexai.

==> sec/0_abstract.tex <==
\begin{abstract}

\end{abstract}

==> sec/Archive/1_intro.tex <==
\section{Introduction}

% Lack of XAI metrics survey dedicated to object detection models

% Shortcomings of previous XAI metrics/surveys:
% - Applicability of each metric for specific XAI methods.

% Research questions:

% Our contributions:

Deep neural networks are increasingly used for object detection in fields such as healthcare \cite{wu2019deep}, autonomous driving \cite{Jia2023}, finance \cite{9092995}, security \cite{10266136}, and visual inspection \cite{10444225, ijcai2024p1025} due to their exceptional performance. However, their lack of transparency raises concerns among end-users and may hinder AI adoption, particularly in trust-sensitive domains. Furthermore, regulations like the European General Data Protection Regulation (GDPR) now mandate greater transparency in the use of AI models. This has driven growing interest in eXplainable Artificial Intelligence (XAI) within the research community.

As XAI solutions become more common and essential, it is crucial to evaluate their explainability components effectively \cite{app12199423}. This evaluation serves multiple purposes, such as verifying that explanations accurately reflect the underlying AI model and ensuring they are useful to end users. Current XAI research primarily focuses on developing new methods to enhance explainability while maintaining high predictive performance. However, some argue that the mere presence of explanations, regardless of their content, can foster a false sense of security \cite{10.1145/3290607.3312787}. Additionally, human bias toward simpler explanations may lead to the adoption of more persuasive outputs over more transparent ones \cite{herman2019promiseperilhumanevaluation}. Therefore, rigorous evaluation of XAI methods is essential both before deployment and throughout their use in production environments.

The multidisciplinary nature of XAI systems introduces challenges in developing effective methodologies for their evaluation. Current efforts to quantitatively validate XAI methods face several shortcomings, which this work aims to address:
% Continue to read and paraphrase from here
% Ref 1: Navigating the Maze of Explainable AI: A Systematic Approach to Evaluating Methods and Metrics
% Ref 2: XAI Systems Evaluation: A Review of Human and Computer-Centred Methods
\begin{itemize} 
    \item \textbf{Lack of consensus}: % Only take idea from Ref 1

    \item \textbf{Lack of standardized evaluation procedures}: % Only take idea Ref 2 

    \item \textbf{Individual XAI metrics lack trustworthiness}: % Only take idea from Ref 1
\end{itemize}

% Should we add some RQs as in Ref 1 or go straight to contributions?


:

==> sec/Archive/2a_background.tex <==
\section{Background}
% Write something to summarize this section
\subsection{Object Detection Models}
% *** Contents: 
% - Faster-RCNN, YOLO family
% *** Notes:
% - Illustrative figures for the architectures (if have enough space)?
% *** References:
% - Comprehensive summary tables: https://www.sciencedirect.com/science/article/abs/pii/S1051200422004298
% - Comprehensive figure 1 for 1 and 2 stage detectors: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8825470
% - Other: https://arxiv.org/pdf/2104.11892
% - Other: https://arxiv.org/pdf/1807.05511#page=3.07

Object detection involves identifying and locating objects in an image, typically using rectangular bounding boxes to indicate their positions and detection confidence \cite{l1}. Advances in deep learning and computational power have significantly enhanced this field. For example, deep convolutional neural networks, well-known for their strong feature representation, are now commonly used in object detection models \cite{l2, l3}. Detection methods are generally classified as either two-stage or one-stage. Two-stage detectors first generate region proposals and then classify them into object categories. In contrast, one-stage detectors predict object categories and locations in a single step, treating detection as a regression or classification task \cite{l1, l2, l3, l4}.

A two-stage detector, also known as a region proposal-based framework, generates region proposals through a dedicated module \cite{l5}. In the first stage, the model detects object proposals, which are then classified and localized in the second stage. This approach offers high detection accuracy but often results in complex architectures, slower proposal generation, and limited global context \cite{l3, l4}. Key examples of two-stage detectors include R-CNN (Region-based Convolutional Neural Network) \cite{l6}, Fast R-CNN \cite{l7}, Faster R-CNN \cite{l8}, and Mask R-CNN \cite{l9}.

One-stage detectors, or one-shot detectors, eliminate the region proposal phase by directly predicting object locations and categories in a single step. This approach enhances detection speed and is ideal for real-time applications, balancing efficiency with acceptable accuracy. Prominent examples include YOLO (You Only Look Once) \cite{l14, l16, l17, l19, l22} and SSD (Single Shot Multibox Detector) \cite{l15}. Their end-to-end design enables fast inference, though accuracy may decline when detecting small objects or analyzing complex scenes.

% In this paper, a model ... will be used

\subsection{XAI Methods for Object Detection} 
XAI in object detection focuses on interpreting spatial and feature-level contributions that influence model predictions. It helps identify false detections, understand occlusion effects, and reveal biases in model behavior. XAI methods are generally classified by their explanation techniques, including perturbation-based, backpropagation-based, Class Activation Mapping (CAM)-based, and example-based approaches \cite{journalpaper}.

In this paper, we will employ 11 XAI methods. Specifically, for perturbation-based approaches, we apply D-RISE (Detector Randomized Input Sampling for Explanation) \cite{Petsiuk2021drise}, D-CLOSE (Detector-Cascading multiple Levels of Segments to Explain) \cite{pmlr-v222-truong24a}, FSOD (Fast Shapley-based Object Detection) \cite{10445187}, and BSED (Baseline Shapley-based Explainable Detector) \cite{10505291}. For backpropagation-based methods, we use LRP (Layer-wise Relevance Propagation) \cite{kohlbrenner2020bestpracticeexplainingneural, dreyer2021xai} and DeepLIFT (Deep Learning Important FeaTures) \cite{shrikumar2019learningimportantfeaturespropagating, dreyer2021xai}. CAM-based methods include ODAM (Object Detector Activation Maps) \cite{10478163}, G-CAME (Gaussian Class Activation Mapping Explainer) \cite{nguyen2023gcamegaussianclassactivationmapping}, SS-Grad-CAM (Spatial Sensitive Grad-CAM) \cite{9897350}, and SS-Grad-CAM++ (Spatial Sensitive Grad-CAM++) \cite{Yamauchi_2024_CVPR}. Example-based methods are not considered, as they are less prominent in object detection tasks.

\subsection{Evaluation Metrics for Explainable Object Detection} 
As the variety and availability of XAI methods continue to grow, ensuring their reliability is essential \cite{NEURIPS2018_294a8ed2}. The trustworthiness of these methods is typically evaluated based on six key criteria: how accurately they reflect model reasoning (``Faithfulness''), their consistency under small variations (``Robustness''), their focus on relevant regions (``Localisation''), the clarity of their explanations (``Complexity''), their responsiveness to model or data changes (``Randomisation''), 
and their compliance with established theoretical principles (``Axiomatic'') \cite{JMLR:v24:22-0142}. 
While qualitative assessments, such as saliency map evaluations \cite{doshivelez2017rigorousscienceinterpretablemachine, 10.1145/2939672.2939778, pmlr-v70-shrikumar17a}, can be subjective and difficult to scale, numerous quantitative metrics have been developed to measure XAI methods against these six criteria \cite{klein2025navigatingmazeexplainableai}.

This paper focuses on metrics from the "Faithfulness" and "Localisation" categories to align with object detection tasks. In total, we utilize seven metrics. For "Faithfulness," we apply Sanity Check \cite{NEURIPS2018_294a8ed2, padmanabhan2023sanitycheckssaliencymethods}, Average Drop and Average Increase \cite{chattopadhay2018grad}, Deletion and Insertion \cite{deletion}, and D-Deletion \cite{ddeletion}. In the "Localisation" category, we use Pointing Game \cite{pointinggame}, EBPG (Energy-based Pointing Game) \cite{wang2020score}, and VEA (Visual Explanation Accuracy) \cite{oramas2018visual}.



==> sec/Archive/2b_related_work.tex <==
\section{Related Work}
Previous Surveys for XAI Evaluation Metrics
=> Not yet: Metrics for object detection models 

==> sec/Archive/3_survey_methodology.tex <==
\subsection{Survey Methodology}
Describe how we find for XAI methods/metrics for object detection models, count the number of times that metrics being used.

Keyword (XAI methods, metrics, object detection) => how many papers using these metrics, source, year-year (all).

\subsection{Fundamental Concepts and Notations}
This part defines the basic concepts and notations used in our discussion of AI-based technologies. Since XAI methods and evaluation metrics often stem from diverse sources with varying terminologies, we establish a unified notation system to ensure consistency and clarity throughout. A summary is provided in \autoref{nota}.

\begin{table*}[ht!]
\centering
\caption{Summary of key concepts and notations}
\label{nota}
\begin{tabularx}{\textwidth}{@{} L{0.3} L{0.3} L{0.4} L{1} @{}}
\toprule
\textbf{Concept} & \textbf{Notation} & \textbf{Expression} & \textbf{Description} \\ \midrule

Input set & \centering $\mathcal{X}$ & $\mathcal{X} = \{\bold{x}_1, \cdots, \bold{x}_n \}$ & The set of all input instances, where each input $\bold{x} \in \mathcal{X}$ can be in the form of text, tabular data, or an image, and is represented as an array for model processing. \\ \addlinespace

Target set & \centering $\mathcal{Y}$ & $\mathcal{Y} = \{y_1, \cdots, y_n \}$ & The set of all target values or labels, where each $y \in \mathcal{Y}$ represenzts the ground truth for an input $\bold{x} \in \mathcal{X}$, and  can be in scalar or array form, depending on the nature of the task. \\ \addlinespace

Output set & \centering $\hat{\mathcal{Y}}$ & $\hat{\mathcal{Y}} = \{\hat{y}_1, \cdots, \hat{y}_n \}$ & The set of all output values, where each $\hat{y} \in \hat{\mathcal{Y}}$ corresponds to the model's output for an input $\bold{x} \in \mathcal{X}$, and  can be in scalar or array form, depending on the nature of the task. \\ \addlinespace

Explainer & \centering $e$ & $e: \mathcal{X} \rightarrow \mathcal{E}$ & The mapping $e: \mathcal{X} \rightarrow \mathcal{E}$ defines an explanation function, where each input $\bold{x} \in \mathcal{X}$ is mapped to a generated explanation $e(\bold{x}) \in \mathcal{E}$. This explanation provides insights, such as feature importance or decision logic, to clarify how the model responds to each input. \\ \addlinespace

Predictor & \centering $f$ & $f: \mathcal{X} \rightarrow \hat{\mathcal{Y}}$ & The mapping $f: \mathcal{X} \rightarrow \hat{\mathcal{Y}}$ defines a prediction function, where each input $\bold{x} \in \mathcal{X}$ is mapped to a predicted output $\hat{y} \in \hat{\mathcal{Y}}$. The function is trained to approximate the true target $y \in \mathcal{Y}$ for a specific learning task. \\ \addlinespace

Bounding box & \centering $\bold{b}$ & $\bold{b}=\left[\bold{L}, O, \hat{y} \right]$ & Represents a bounding box proposal where $\bold{L}$ denotes the coordinates (e.g., top-left and bottom-right corners), $O$ is the objectness score indicating the confidence that an object is present, and $\hat{y}$ is the predicted class label associated with the bounding box. \\ \addlinespace

\bottomrule
\end{tabularx}
\end{table*}

==> sec/Archive/4_methods_metrics.tex <==
(same post-modeling, local, posthoc => explain) => pre/in-/post, local/global... 

\section{XAI Methods for Object Detection}\todo[]{May skip the above table. Rewrite all methods/metrics using only words in short paras. Take SS-GradCam as example}
% Write a brief intro here

\subsection{Perturbation-based}
\begin{comment}
  \begin{enumerate}
    \item D-RISE:

    \item D-CLOSE:

    \item BSED: % https://www.researchgate.net/publication/379966671_BSED_Baseline_Shapley-Based_Explainable_Detector
    
    \item FSOD: % https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10445187

\end{enumerate}  
\end{comment}

\subsubsection{Detector Randomized Input Sampling for Explanation (D-RISE)} 
D-RISE \cite{Petsiuk2021drise} explains object detectors by generating saliency maps through random binary masking of input images. The detector’s response to each masked image is compared to the target detection using a similarity metric that considers bounding box overlap (IoU), class probabilities, and objectness scores. The highest-scoring detection for each mask is selected, and the final saliency map is produced by weighting and summing these masks based on their alignment with the target.

\subsubsection{Detector-Cascading multiple Levels of Segments to Explain (D-CLOSE)} 
D-CLOSE \cite{pmlr-v222-truong24a} explains object detection models by generating saliency maps through cascading multi-level segmentation of input images. It uses Simple Linear Iterative Clustering (SLIC) to create random perturbation masks, capturing both fine and coarse features. Masked images are processed by the detector, and predictions are weighted based on their similarity to the target using Intersection over Union (IoU) and class probabilities. A density map normalizes these results to correct uneven mask distribution, which helps reduce noise and sharpening explanations. The method fuses feature maps from different segmentation levels, prioritizing finer details for improved localization and classification.

\subsubsection{Fast Shapley-based Object Detection (FSOD)} 
FSOD \cite{10445187} introduces a real-time explainability framework for object detection by training an explainer model to estimate Shapley values directly from feature maps. This avoids the high computational cost of traditional sampling and perturbation methods. The method defines a detection-specific value function that integrates objectness, classification confidence, and Intersection over Union (IoU) to reflect both localization and classification. FSOD employs a UNet-based architecture to process multi-scale feature maps, ensuring precise spatial representation across detection layers. A query map provides object-specific context, guiding the explainer to focus on individual detections. This enables FSOD to generate saliency maps that align closely with object boundaries.

\subsubsection{Baseline Shapley-based Explainable Detector (BSED)} 
BSED \cite{10505291} applies Shapley values to object detection, producing saliency maps that attribute detection outputs to image regions. It perturbs input images with binary masks, evaluates detection results, and aggregates feature attributions while maintaining key properties like efficiency and linearity. To reduce the high computational cost of exact Shapley calculations, BSED uses a multilayer approximation that samples masks at different ratios. The method captures both positive and negative contributions, offering deeper insights into model behavior.

\subsection{Backpropagation-based}
\begin{comment}
  \begin{enumerate}
    \item LRP: % https://www.maxdreyer.de/static/xai_comparison_dreyer-b5704c4c44a709e1a9e37cd9173e85ae.pdf#page=4.69
    \item DeepLIFT: % https://www.maxdreyer.de/static/xai_comparison_dreyer-b5704c4c44a709e1a9e37cd9173e85ae.pdf#page=4.69
\end{enumerate}  
\end{comment}

\subsubsection{Layer-wise Relevance Propagation (LRP)}
LRP \cite{kohlbrenner2020bestpracticeexplainingneural} explains how neural networks make predictions by redistributing output scores across input features, layer by layer, while preserving the principle of relevance conservation. In object detection, LRP traces relevance from the final output back through the network, identifying the contribution of each input pixel to bounding box predictions \cite{dreyer2021xai}. For SSD (Single Shot Detector) models, LRP is adjusted to handle $l_2$-Norm layers by treating them as activation functions, which ensures stable and consistent relevance propagation. Additionally, various propagation rules are applied to balance noise suppression and feature sensitivity. LRP enhances feature localization and sharpens object boundaries, leading to more accurate bounding box predictions and improved overall interpretability.

\subsubsection{Deep Learning Important FeaTures (DeepLIFT)}
DeepLIFT \cite{shrikumar2019learningimportantfeaturespropagating} explains neural network predictions by comparing the difference between a neuron’s activation and its reference state to assess the influence of input features. In object detection, DeepLIFT tracks how intermediate neuron activations deviate from a baseline, often a blurred version of the input, to determine the contribution of each pixel to bounding box predictions \cite{dreyer2021xai}. The method propagates contribution scores backward through the network using the chain rule, similar to backpropagation. For nonlinear layers, the Rescale rule is applied, ensuring relevance is distributed proportionally to activation changes. Additionally, the $\gamma$-rule (adapted from LRP) is applied to enhance positive contributions and suppress contradicting signals, resulting in clearer and less noisy heatmaps. DeepLIFT allows for detailed visualization of small-scale features and achieves efficient computation with a single forward and backward pass.

\subsection{Class Activation Mapping (CAM)-based}
\begin{comment}
\begin{enumerate}
    \item ODAM: % https://github.com/Cyang-Zhao/ODAM CAM-based
    \item G-CAME: https://www.cs.unb.ca/~hcao3/publications/2024-canadianai/GCAME_CANAI_Presentation.pdf, https://arxiv.org/abs/2306.03400 -> Done
    \item SS-GradCAM: % https://ieeexplore.ieee.org/abstract/document/9897350
    \item SS-GradCAM++: % https://openaccess.thecvf.com/content/CVPR2024W/XAI4CV/html/Yamauchi_Spatial_Sensitive_Grad-CAM_Improved_Visual_Explanation_for_Object_Detectors_via_CVPRW_2024_paper.html
\end{enumerate}    
\end{comment}

\subsubsection{Object Detector Activation Maps (ODAM)}
ODAM \cite{10478163} explains object detection results by generating instance-specific heat maps. It calculates the gradients of prediction attributes, like class scores and bounding box coordinates, with respect to the detector’s feature maps. These gradients are computed at each pixel to identify which regions influence the detection. Unlike Grad-CAM \cite{Selvaraju_2019}, ODAM preserves fine spatial details by keeping gradients at the pixel level rather than averaging them. The gradients are smoothed, applied to feature activations, and produce heat maps that show the most important areas for each detection. This method provides distinct, instance-level explanations, avoiding the overlap and ambiguity seen in class-specific approaches. ODAM is compatible with one-stage, two-stage, and transformer-based detectors, and can generate high-quality visualizations with minimal computational cost.

\subsubsection{Gaussian Class Activation Mapping Explainer (G-CAME)}
G-CAME ~\cite{nguyen2023gcamegaussianclassactivationmapping} explains object detection by generating saliency maps using gradients and Gaussian masking. First, the gradient map $G^{l(c)}_k = \partial S^c/\partial A_k^l$ is calculated, where $l$ is the selected convolutional layer, $S^c$ is the target class score, and $A_k^l$ is the feature map. Then, the feature maps are weighted by their corresponding gradient values and split into positive contributions $A_{k_1}^{c(+)}$ (enhancing the target score) and negative contributions $A_{k_2}^{c(-)}$ (reducing the score). To localize the explanation, a Gaussian mask $G_\sigma$ is used:
\begin{align}
G_\sigma = \displaystyle \frac{1}{2\pi\sigma^2} \exp \bigg(-\displaystyle \frac{d_i^2+d_j^2}{2\sigma^2} \bigg),
\end{align}
where $(d_i,d_j)$ are distances from the object center and $\sigma$ determines the focus area around the object. Finally, the saliency map is computed as:
\begin{align}
L_\text{G-CAME}^c = \text{ReLU} \left( \sum_{k_1} G_\sigma(k_1) \odot A_{k_1}^{c(+)}  - \sum_{k_2} G_\sigma(k_2) \odot A_{k_2}^{c(-)} \right).
\end{align}
Here, $G_\sigma$ serves as a weighting factor for each pixel in the weighted feature maps, which helps emphasize object-relevant regions while suppressing irrelevant areas and noise.

\subsubsection{Spatial Sensitive Grad-CAM (SS-Grad-CAM)} 
SS-Grad-CAM \cite{9897350} enhances Grad-CAM \cite{Selvaraju_2019} by addressing its lack of spatial precision, which often causes heatmaps to highlight irrelevant areas. Key features of SS-Grad-CAM include space maps, which are created by normalizing the absolute gradients of detection scores with respect to feature maps. These maps highlight regions with the highest gradient responses, ensuring heatmaps focus on areas directly influencing detection. Applying space maps to feature maps reduces activations in unrelated regions, producing sharper and more accurate visual explanations. 

\subsubsection{Spatial Sensitive Grad-CAM++ (SS-Grad-CAM++)} 
SS-Grad-CAM++ \cite{Yamauchi_2024_CVPR} improves visual explanations for object detectors by enhancing the calculation of feature importance and spatial relevance. First, it computes feature importance by combining gradients of the detection score with respect to the feature map $A^k$. The importance weights $w_k^{c,\text{det}}$ are derived using a weighted combination of the first, second, and third-order derivatives of $\hat{y}^c_\text{det}$, providing a more accurate measure of contribution. Then, a binary mask $M^{k,\text{det}}$ is employed to identify regions relevant to the detected instance, such as ROI pooling or bounding boxes. To account for spatial relevance, SS-Grad-CAM++ normalizes gradient magnitudes to create a space map $S^{c,\text{det}}_k$, which emphasizes the most influential neurons. The final heat map $L^{c,\text{det}}$ is generated by combining the feature importance and space map through element-wise multiplication, followed by a ReLU operation to eliminate negative contributions.

\section{XAI Evaluation Metrics for Object Detection}
\subsection{Faithfulness}
% Sanity check: https://arxiv.org/pdf/2306.02424#page=1.63 -> Done; revise to shorten
% Decrease/Increase: -> Done
% Deletion/Insertion: -> Done; (revise to insert formula)

\subsubsection{Sanity Check} 
Sanity check \cite{NEURIPS2018_294a8ed2, padmanabhan2023sanitycheckssaliencymethods} evaluates the reliability of saliency-based explanations in deep learning models. Originally developed for general saliency evaluations, it was later adapted for object detection tasks. The metric consists of two tests. The Model Randomization Test evaluates whether saliency maps are sensitive to changes in model parameters. It qualitatively compares maps from a trained model ($\bold{S}_T$) and a model with randomized weights ($\bold{S}_R$) using the Structural Similarity Index Measure (SSIM), defined as
\begin{align}
\text{SSIM}(S_{\text{T}}, S_{\text{R}}) = \frac{(2\mu_S\mu_T + C_1)(2\sigma_{ST} + C_2)}{(\mu_S^2 + \mu_T^2 + C_1)(\sigma_S^2 + \sigma_T^2 + C_2)}
\end{align}
where $\mu_S$, $\mu_T$ represent the mean pixel intensities of $\bold{S}_T$ and $\bold{S}_R$; $\sigma_S^2$, $\sigma_T^2$ are the variances; $\sigma_{ST}$  denotes the covariance; and $C_1$, $C_2$ are constants for numerical stability. A low SSIM score indicates high sensitivity, meaning the explanation method effectively reflects model parameters. The Data Randomization Test assesses whether saliency maps distinguish between models trained on correct labels and those trained on random labels. It qualitatively examines the maps for differences in focus, texture, and intensity. If the maps from both cases are similar, the explanation method is considered ineffective, as it fails to capture meaningful input-label relationships.

\subsubsection{Average Drop and Average Increase} 
Average Drop and Average Increase metrics \cite{chattopadhay2018grad} evaluate the effectiveness of saliency maps in identifying critical regions for model predictions:
\paragraph{\textbf{Average Drop (\%)}} measures the percentage decrease in the model’s confidence for the target class when only the highlighted regions are retained:
\begin{align}
    \text{Average Drop} = \frac{1}{N} \sum_{i=1}^N \max\left(0, \frac{\hat{y}^c_i - \hat{y'}^c_i}{\hat{y}^c_i}\right) \times 100
\end{align}
where: $\hat{y}^c_i$ is the confidence for class $c$ on the original image $i$; $\hat{y'}^c_i$ denotes the confidence with only the highlighted regions retained, and; $N$ presents the total number of images. Lower values indicate better explanations.   

\paragraph{\textbf{Average Increase (\%)}} computes the proportion of cases where retaining only the highlighted regions increases confidence:
\begin{align}
    \text{Average Increase} = \frac{1}{N} \sum_{i=1}^N \text{sign}\Big(\hat{y}^c_i < \hat{y'}^c_i\Big)
\end{align}
where: $\text{sign}(\cdot)$ presents an indicator function that returns 1 if the input is True and 0 otherwise. Higher values reflect better explanations.


\subsubsection{Deletion and Insertion}
Deletion and Insertion metrics \cite{deletion} evaluate the quality of saliency maps by measuring their ability to identify regions critical for a model's prediction. In the Deletion metric, pixels ranked as most important in the saliency map are progressively removed from the input image, and the drop in the target class probability is recorded. Conversely, the Insertion metric adds important pixels back to a blurred baseline image, recording the rise in the target probability. Both metrics generate a curve of probability versus pixel fraction, and the area under the curve (AUC) serves as the performance measure. A lower AUC in Deletion and a higher AUC in Insertion indicate better explanation quality.

\paragraph{D-Deletion}
D-Deletion metric \cite{ddeletion} extends the standard Deletion metric \cite{deletion} by adding spatial localization, making it more effective for object detection tasks. The metric operates on image data, specifically targeting inputs in the form of saliency maps generated by object detection models. As a result, it is compatible with saliency-based XAI methods. Mathematically, D-Deletion is defined as:
\begin{align}
\text{D-Deletion}(\bold{x}, \bold{S}, y) = \text{AUC} \left( \left\{ \max_{\bold{b}_j^k} \left[ O_j^k \cdot \mathbb{I}(\hat{y}_j^k = y) \cdot \mathbb{I}(\text{IoU}(\bold{b}, \bold{b}_j^k) > \gamma) \right] \right\}_{k=1}^{K} \right)
\end{align}
where
\begin{itemize}
    \item $\bold{S}$ identifies the saliency map produced by an XAI method;
    \item $\text{AUC}(\cdot)$ is the Area Under the Curve metric;
    \item $K$ represents the total number of deletion steps;
    \item $j$ is the index of a predicted bounding box at masking step $k$;
    \item $\mathbb{I}(\hat{y}_j^k = y)$ functions as an indicator, returning 1 if the predicted class $\hat{y}_j^k$ matches the target class $y$, and 0 otherwise, and;
    \item $\mathbb{I}(\text{IoU}(\bold{b}, \bold{b}_j^k) > \gamma)$ acts as an indicator that equals 1 if the IoU between the ground truth box $\bold{b}_j^k$ and the detected box $\bold{b}$ exceeds the threshold $\gamma$, and 0 otherwise.
\end{itemize}
D-Deletion metric works as follows: the most influential pixels identified by a saliency map are progressively masked out. After each deletion, the model re-evaluates the masked image to produce updated bounding box predictions. The metric considers only bounding boxes that match the target class and have an Intersection over Union (IoU) above a specified threshold with the ground truth box. At each step, it tracks the highest confidence score among these bounding boxes, and the area under the curve (AUC) of these scores measures the drop in confidence. A lower AUC indicates that the masked regions were critical for both classification and localization, thus validating the accuracy of the saliency map.

\subsection{Localization}
%... (known as Plausibility)
% Pointing Game (PG) -> Done
% Energy-based Pointing Game (EBPG) -> Done; revise to shorten
% IoU (maybe they call VEA in this paper: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=\&arnumber=10445187) -> Done; revise to add formula

\subsubsection{Pointing Game}
The Pointing Game metric \cite{pointinggame} assesses the spatial localization performance of XAI techniques, independently of the model’s classification accuracy. The core idea is to evaluate whether the highest activation point in the saliency map falls within the ground-truth bounding box of the target object. The accuracy of the Pointing Game is calculated as
\begin{align}
\text{Accuracy} = \displaystyle \frac{\# \text{hits}}{\#\text{hits} + \# \text{misses}}
\end{align}
A ``hit'' is counted if the highest activation point falls within the ground-truth bounding box of the target object; otherwise, it is a ``miss.'' The accuracy score is averaged over all evaluated categories.

\subsubsection{Energy-based Pointing Game (EBPG)}
The EBPG metric \cite{wang2020score} evaluates the quality of saliency maps produced by XAI methods in object detection models. Its purpose is to assess how well the saliency map identifies the regions in the image that contain the object of interest. The input to EBPG includes a saliency map and ground truth bounding boxes. The output is a score between 0 and 1, where a higher score indicates better localization accuracy.

EBPG works by calculating the fraction of the saliency values within the bounding box relative to the total saliency across the entire image. Mathematically, it is defined as:
\begin{align}
\text{EBPG} =\displaystyle \frac{\sum_{(i, j) \in \bold{b}} S_{\bold{x}, \hat{y}}(i, j)}{\sum_{(i, j) \in \bold{b}} S_{\bold{x}, \hat{y}}(i, j) + \sum_{(i, j) \notin \bold{b}} S_{\bold{x}, \hat{y}}(i, j)}
\end{align}
where
\begin{itemize}
    \item $S_{\bold{x}, \hat{y}}(i, j)$ denotes the saliency score at pixel $(i, j)$;
    \item $\sum_{(i, j) \in \bold{b}} S_{\bold{x}, \hat{y}}(i, j)$ represents the total sum of saliency values inside the bounding box, and;
    \item $\sum_{(i, j) \notin \bold{b}} S_{\bold{x}, \hat{y}}(i, j)$ indicates the total sum of saliency values outside the bounding box.
\end{itemize}

\subsubsection{Visual Explanation Accuracy (VEA)}
The VEA metric \cite{oramas2018visual} evaluates how well an explanation method identifies important regions by comparing saliency maps to ground-truth masks. A threshold is applied to the saliency map to isolate high-importance areas, and the Intersection over Union (IoU) is calculated between these thresholded regions and the ground-truth mask. This process is repeated for a range of thresholds, with IoU values plotted against the thresholds to form a curve. The overall performance is summarized by the area under this curve (AUC).

\subsection{Robustness}
... (optional/mostly for classification)

\subsection{Complexity}
... (optional)
% Running time: 

\subsection{Randomization}
... (optional)





% Include a table for each XAI method, public code?, category, published year, used metrics, categories... (same post-modeling, local, posthoc, images data...)


==> sec/Archive/5_benchmark.tex <==
\section{Framework}
% Include a framework image...

Benchmark methods and metrics on few datasets like MS-COCO validation with FasterRCNN with ResNet50 backbone. (YOLOX later).
% Methodology flow can be like: https://www.researchgate.net/publication/365367673_A_Trustworthy_View_on_XAI_Method_Evaluation
% Qualitative Eval
% Quantitative Eval

% Split MS COCO by size via k-mean https://github.com/Binh24399/D-CLOSE/blob/main/demo.ipynb

\subsection{Qualitative Evaluation}
\subsubsection{Saliency Maps Evaluation}
\subsubsection{Sanity Check}

\subsection{Quantitative Evaluation}
\subsubsection{Faithfulness}
\subsubsection{Localization}
\subsubsection{Running time}


==> sec/XX_test_metric.tex <==
\section{Localization}
The quality of an explanation in the context of localization is measured by how well it aligns with a user-defined region of interest (ROI) \cite{FindingtheRightXAIMethodAGuidefortheEvaluationandRankingofExplainableAIMethodsinClimateScience}. This is done by comparing the positions of the pixels with the highest relevance values, provided by the XAI explanation, to the labeled areas such as bounding boxes or segmentation masks. Since the ROI is assumed to play a key role in the network's decision (ground truth) \cite{FindingtheRightXAIMethodAGuidefortheEvaluationandRankingofExplainableAIMethodsinClimateScience,arras2022clevr,zhang2018top}, an explanation map is considered to have high localization performance if the most relevant pixels are concentrated within the ROI. To quantify localization, we use the Pointing Game \cite{zhang2018top} and Energy-based Pointing Game (EBPG) \cite{wang2020score} metrics.

\subsection{Pointing Game}
Pointing Game (PG) \cite{zhang2018top} evaluates the spatial precision of saliency maps by measuring their ability to localize target object categories. For each saliency map, the metric identifies the point of maximum saliency and checks if it falls within the ground truth annotation of the target object. A hit is recorded if the point lies within the annotated region; otherwise, it is counted as a miss. The localization accuracy is defined as:
\begin{align}
    \text{PG} = \frac{\text{\# Hits}}{\text{\# Hits}+\text{\# Misses}}
\end{align}
where $\text{\# Hits}$ and $\text{\# Misses}$ denote the total number of correct and incorrect localizations, respectively. The overall performance is calculated by averaging the accuracy across all categories. A high Pointing Game score for an XAI method indicates its ability to generate accurate and interpretable saliency maps. 
\begin{comment}
    Pointing Game has two primary strengths: a) it evaluates the spatial selectivity of saliency maps without requiring the entire object to be highlighted or accounting for the CNN model’s classification accuracy, and b) it involves minimal post-processing, which allows for a fairer and more consistent evaluation of different maps.
\end{comment}

\subsection{Energy-Based Pointing Game}
EBPG \cite{wang2020score} evaluates the spatial accuracy of saliency maps by analyzing how much of the map’s energy (activation) falls within the annotated bounding box of the target object. Unlike the traditional Pointing Game, which focuses on a single maximum point, this metric considers the overall distribution of energy within the relevant regions. The localization accuracy is defined as:
\begin{align}
\text{EBPG} = \frac{\sum L^c_{(i,j) \in \text{bbox}}}{\sum L^c_{(i,j) \in \text{bbox}} + \sum L^c_{(i,j) \not\in \text{bbox}}}
\end{align}
where $L^c_{(i,j)}$ represents the saliency map intensity at pixel $(i,j)$, and ``bbox'' refers to the bounding box region of the target object. The overall performance is calculated by averaging the accuracy across all categories. A high EBPG value indicates that the XAI-generated saliency maps can effectively localize the target region and suppress noise outside the bounding box. 
\begin{comment}
    Compared to the traditional Pointing Game, EBPG offers a more holistic and robust evaluation by using the overall energy distribution instead of a single point.
\end{comment}

\section{Faithfulness}
Faithfulness quantifies the impact of altering the number of features assigned high relevance by an explanation method on the model’s prediction \cite{pmlr-v222-truong24a}. This is assessed by incrementally adding or removing input pixels with high relevance values and comparing the resulting predictions to the original ones. Since relevance reflects each feature’s contribution to the prediction, changes in the number of high-relevance features are expected to significantly impact the prediction. To measure Faithfulness, we employ the Deletion and Insertion \cite{petsiuk2018riserandomizedinputsampling}, as well as the Over-All \cite{zhang2021group} metrics.

\subsection{Deletion and Insertion} % add some more metrics?
The Deletion \cite{petsiuk2018riserandomizedinputsampling} metric evaluates the effect of removing key features by tracking the decline in predicted class probability as important pixels, identified by the saliency map, are progressively removed. A steep probability drop, quantified by a low area under the curve (AUC), denotes a strong explanation. In contrast, the Insertion \cite{petsiuk2018riserandomizedinputsampling} metric measures the probability increase when pixels are gradually introduced, with a higher AUC indicating better explanations. 
% Common strategies for pixel removal include replacing values with zero, a constant gray, or applying blurring, while insertion methods involve adding pixels to a blank canvas or progressively unblurring regions. 
% For Insertion,  starting with a blurred canvas reduces spurious artifacts that may mislead the model. For Deletion, constant-value replacement is more effective, as blurred regions often allow robust models to infer missing details from contextual information.

\subsection{Over-All}
The Over-All \cite{zhang2021group} metric, defined as $\text{AUC}(\text{Insertion}) - \text{AUC}(\text{Deletion})$, provides a comprehensive evaluation of saliency map quality by considering both its positive and negative effects on the model’s predictions. A higher score indicates the saliency map effectively highlights critical regions (high Insertion) while minimizing the influence of irrelevant ones (low Deletion).
% which reflects the alignment between the XAI method and the model’s decision-making process.

\section{Complexity}
As stated in \cite{FindingtheRightXAIMethodAGuidefortheEvaluationandRankingofExplainableAIMethodsinClimateScience}, complexity refers to the conciseness of an explanation, which should focus on a small number of key features. Concise explanations, defined by these important features, are easier for researchers to interpret and are likely to offer more valuable information with less noise \cite{FindingtheRightXAIMethodAGuidefortheEvaluationandRankingofExplainableAIMethodsinClimateScience,10.1007/978-3-031-09037-0_8}. Additionally, this work incorporates the computational time of explanation methods into the complexity measure. High computation time can hinder the applicability of XAI methods, especially in real-time applications and complex pipelines \cite{KAKOGEORGIOU2021102520}. To quantify complexity, we use the Sparsity \cite{10.1007/978-3-031-09037-0_8} metric and record the runtime of each XAI method considered.

\subsection{Sparsity}
% This may belong to Faithfulness -> may change to Sparsity/other metric in Quantus
The Sparsity \cite{10.1007/978-3-031-09037-0_8} metric measures how concentrated or dispersed the scores in a saliency map are, reflecting the focus of attention on specific regions. It is defined as the ratio of the maximum score ($S_\text{max}$) to the mean score ($S_\text{mean}$):
\begin{align}
    \text{Sparsity} = \frac{S_\text{max}}{S_\text{mean}}
\end{align}
To ensure consistency across methods, saliency map scores are normalized as:
\begin{align}
    S' = \frac{S-S_\text{min}}{S_\text{max}-S_\text{min}}
\end{align}
This normalization simplifies the metric to:
\begin{align}
    \text{Sparsity} = \frac{1}{S'_\text{mean}}
\end{align}
A high sparsity value corresponds to a high $S_\text{max}/S_\text{mean}$ ratio, i.e., a low mean score $S_\text{mean}$, indicating that the map's focused areas are narrow and well-defined. 
% The metric is sensitive to the distribution of saliency scores and can effectively quantify varying levels of focus within saliency maps.

\subsection{Computation Time}
% State when to start and when to stop + why + notes
This metric records the time taken to compute explanations for a given model input. It is typically reported as the average runtime per instance and depends on factors such as model complexity, input size, and explanation method. Lower values indicate higher efficiency, while higher values reflect greater computational cost.

\subsection{D-CLOSE}
D-CLOSE \cite{pmlr-v222-truong24a} generates saliency maps by segmenting the input image at multiple levels and combining their features to enhance explanation quality. Random masks are used to perturb the input, and the similarity scores between the masked outputs and the target prediction are calculated to weigh the importance of each region. The saliency maps are normalized using a density map to reduce noise, and multi-scale feature fusion aggregates fine-grained to coarse-grained features. 

\subsection{D-RISE}
D-RISE \cite{Petsiuk_2021_CVPR} is a black-box attribution method developed to generate saliency maps for object detectors. It explicitly considers both the localization and classification aspects of detection. The method applies randomized binary masks to the input image and assesses their influence on detection outcomes. Each masked region’s importance is evaluated using a similarity metric that combines Intersection over Union (IoU) for spatial overlap, cosine similarity for classification consistency, and objectness scores. The final saliency map is constructed by aggregating masks according to their calculated contributions. 
% A key strength of D-RISE is its effective compatibility with both one-stage and two-stage models.

\subsection{G-CAME}
G-CAME \cite{nguyen2024efficientconciseexplanationsobject} improves CAM-based explanation methods for object detection by integrating a Gaussian kernel for saliency map refinement. Specifically, it combines gradient-based localization with Gaussian weighting, effectively suppressing background noise and enhancing the detection of small objects. The method consists of four steps: selection of target layers, gradient-based object localization, feature map weighting, and Gaussian masking. 
\begin{comment}
    G-CAME \cite{nguyen2024efficientconciseexplanationsobject} enhances CAM-based explanation methods for object detection by integrating a Gaussian kernel for saliency map refinement. Specifically, it combines gradient-based localization with Gaussian weighting to better highlight targeted objects and reduce background interference. This also helps G-CAME work well with tiny objects. The method involves four key steps: selection of target layers, gradient-based object localization, feature map weighting, and Gaussian masking. A notable advantage of G-CAME is its effectiveness in explaining tiny objects.

    G-CAME enhances CAM-based explanation methods for object detection by integrating a Gaussian kernel into saliency map refinement. Conventional CAM approaches often produce noisy saliency maps and lack precision when identifying individual objects. To address these limitations, G-CAME combines gradient-based localization with Gaussian weighting, effectively highlighting targeted objects and reducing background interference. The proposed method involves four key steps: selection of target layers, gradient-based object localization, feature map weighting, and Gaussian masking. Experimental results demonstrate that G-CAME substantially improves the quality of explanations, particularly for very small objects.
\end{comment}
